OSWorld-MCP: Benchmarking MCP Tool Invocation In Computer-Use Agents

With advances in decision-making and reasoning capabilities, multimodal agents show strong potential in computer application scenarios. Past evaluations have mainly assessed GUI interaction skills, while tool invocation abilities, such as those enabled by the Model Context Protocol (MCP), have been largely overlooked. Comparing agents with integrated tool invocation to those evaluated only on GUI interaction is inherently unfair. We present OSWorld-MCP, the first comprehensive and fair benchmark for assessing computer-use agents' tool invocation, GUI operation, and decision-making abilities in a real-world environment. We design a novel automated code-generation pipeline to create tools and combine them with a curated selection from existing tools. Rigorous manual validation yields 158 high-quality tools (covering 7 common applications), each verified for correct functionality, practical applicability, and versatility. Extensive evaluations of state-of-the-art multimodal agents on OSWorld-MCP show that MCP tools generally improve task success rates (e.g., from 8.3% to 20.4% for OpenAI o3 at 15 steps, from 40.1% to 43.3% for Claude 4 Sonnet at 50 steps), underscoring the importance of assessing tool invocation capabilities. However, even the strongest models have relatively low tool invocation rates, Only 36.3%, indicating room for improvement and highlighting the benchmark's challenge. By explicitly measuring MCP tool usage skills, OSWorld-MCP deepens understanding of multimodal agents and sets a new standard for evaluating performance in complex, tool-assisted environments. Our code, environment, and data are publicly available at https://osworld-mcp.github.io.

==> iclr2026/tables/main-result-50steps.tex <==
\begin{table*}[htbp]
\centering
\caption{Performance on OSWorld-MCP (50 Steps).}
\resizebox{\textwidth}{!}{
\begin{tabular}{l l c lll lll lll}
\toprule
\multirow{2}{*}{\textbf{Agent Model}} & 
\multirow{2}{*}{\textbf{Actions}} & \multirow{2}{*}{\textbf{Steps}} & 
\multicolumn{3}{c}{\textbf{Tool-Beneficial Tasks}} & 
\multicolumn{3}{c}{\textbf{Non-Tool-Beneficial Tasks}} & 
\multicolumn{3}{c}{\textbf{Overall}} \\
& & & 
\multicolumn{1}{c}{\textbf{Accuracy}} & \multicolumn{1}{c}{\textbf{TIR}} & \multicolumn{1}{c}{\textbf{ACS}} & 
\multicolumn{1}{c}{\textbf{Accuracy}} & \multicolumn{1}{c}{\textbf{TIR}} & \multicolumn{1}{c}{\textbf{ACS}} & 
\multicolumn{1}{c}{\textbf{Accuracy}} & \multicolumn{1}{c}{\textbf{TIR}} & \multicolumn{1}{c}{\textbf{ACS}} \\
\midrule
\multicolumn{12}{c}{\textit{Open Models}} \\
\midrule
\multirow{2}{*}{Qwen2.5-VL} 
 & GUI & 50 & 12.3 & - & 30.6 & 17.7 & - & 30.4 & 13.9 & - & 30.5 \\
 & + MCP & 50 & 11.7$_{\;0.6\downarrow}$ & 7.3 & 38.6$_{\;8.0\uparrow}$ & 21.6$_{\;3.9\uparrow}$ & 18.9 & 34.2$_{\;3.8\uparrow}$ & 14.8$_{\;0.9\uparrow}$ & 10.9 & 37.2$_{\;6.7\uparrow}$  \\
\multirow{2}{*}{Qwen3-VL} 
 & GUI & 50 & 31.9 & - & 25.5 & 38.0 & - & 25.7 & 33.8 & - & 25.6 \\
 & + MCP& 50 & 37.0 $_{{\;5.1\uparrow}}$ & 27.7 & 20.2$_{{\;5.3\downarrow}}$ & 43.8$_{{\;5.8\uparrow}}$ & 33.3 & 23.3$_{{\;2.4\downarrow}}$ & 39.1$_{{\;5.3\uparrow}}$ & 29.5 & 21.1$_{{\;4.5\downarrow}}$ \\
\midrule
\multicolumn{12}{c}{\textit{Proprietary Models}} \\
\midrule
\multirow{2}{*}{Gemini-2.5-Pro} 
 & GUI & 50 & 11.5 & - & 39.7 & 17.5 & - & 41.7 & 13.3 & - & 40.3  \\
 & + MCP & 50 & 29.5$_{\;18.0\uparrow}$ & 23.2 & 25.2$_{\;14.5\downarrow}$ & 21.6$_{\;4.1\uparrow}$ & 17.7 & 40.2$_{\;1.5\downarrow}$ & 27.2$_{\;13.9\uparrow}$ & 21.5 & 29.7$_{\;10.6\downarrow}$ \\
\multirow{2}{*}{OpenAI o3} 
 & GUI & 50 & 10.7 & - & 43.9 & 17.4 & - & 46.8 & 12.8 & - & 44.8 \\
 & + MCP & 50 & 28.9$_{\;18.2\uparrow}$ & 24.8 & 27.0$_{\;16.9\downarrow}$ & 16.8$_{\;0.6\downarrow}$ & 12.3 & 43.7$_{\;3.1\downarrow}$ & 25.2$_{\;12.4\uparrow}$ & 21.0 & 32.1$_{\;12.7\downarrow}$ \\
\multirow{2}{*}{Seed1.5-VL} 
 & GUI & 50 & 31.2 & - & 22.4 & 40.2 & - & 26.8 & 34.0 & - & 23.8 \\
 & + MCP & 50 & 36.1$_{{\;4.9\uparrow}}$ & 22.7 & 20.8$_{{\;1.6\downarrow}}$ & 43.6$_{{\;3.4\uparrow}}$ & 43.2 & 27.8$_{{\;1.0\uparrow}}$ & 38.4$_{{\;4.4\uparrow}}$ & 29.0 & 23.0$_{{\;0.8\downarrow}}$ \\
\multirow{2}{*}{Claude-4-Sonnet} 
 & GUI & 50 & 38.2 & - & 24.2 & 44.1 & - & 25.6 & 40.1 & - & 24.7 \\
 & + MCP& 50 & 42.4$_{{\;4.2\uparrow}}$ & 35.3 & 18.8$_{{\;5.4\downarrow}}$ & 45.5$_{{\;1.4\uparrow}}$ & 38.7 & 22.8$_{{\;2.8\downarrow}}$ & 43.3$_{{\;3.2\uparrow}}$ & 36.3 &  20.1$_{{\;3.6\downarrow}}$ \\
\midrule
\multicolumn{12}{c}{\textit{Multi-agent Models}} \\
\midrule
\multirow{2}{*}{Agent-S2.5} 
  & GUI & 50 & 46.9 & - & 21.1 & 47.3 & - & 8.4 & 47.1 & - & 20.2 \\
 & + MCP & 50 & 49.4$_{{\;2.5\uparrow}}$ & 32.9 & 16.3$_{{\;4.8\downarrow}}$ & 49.6$_{{\;2.3\uparrow}}$ & 40.5 & 18.7$_{{\;0.3\uparrow}}$ & 49.5$_{{\;2.4\uparrow}}$ & 35.3 & 17.0 $_{{\;3.2\downarrow}}$  \\  \\
\bottomrule
\end{tabular}
}
\label{table:main-results-50}
\end{table*}

